The concentration game: Bayesian updating, regret, and information

We give a two-player zero-sum repeated game between a learner and nature whose value identity generates Bayesian updating and an exact accounting of exponential-weights regret at once, and supplies the comparator-class variational form that a wide class of concentration phenomena share. The terminal payoff is the most a comparator can gain at fixed relative entropy from the prior, and the one-step constraint is an information budget on nature's move under the learner's mixed action. With the learner's move otherwise unrestricted, Gibbs/Bayes weights emerge as its unique Bellman equalizer -- the mixed action that makes the per-round loss independent of which direction nature moves -- with log-partition functions playing the role of value functions. The regret decomposes exactly into three parts: a per-round information loss reflecting the variation in observed outcomes, an additive retempering drift that accounts exactly for any change of measurement scale between rounds, and the information the comparator carries relative to the prior. The variance and bounded-range proxies that drive standard regret bounds are looser relaxations of this decomposition, which holds generally and governs them all. Both players' strategies are read off from the decomposition term by term, and repeated play yields an information-theoretic ledger of self-play in place of the usual quadratic-variation surrogate. The same comparator-class geometry accounts for the classical large-deviation bounds, and methods across bandits, posterior sampling, aggregation, and boosting are specializations of the one regret decomposition.

==> concentration_game_eval.tex <==
% Eval aggregator for concentration_game (P08). Includes per-experiment fragments under eval/E*.tex.
%
% per-experiment fragments under eval/. The main paper includes this with
% a single \input{concentration_game_eval} at the end of the appendix.
%
% Status (2026-05-14). Wave 1 (synthetic, P08-owned): eight fragments all
%
%
% any caveats; individual experiments' frontmatter mirror the same caveats.
%
% No cpu_real or gpu fragments have shipped for P08 yet; this aggregator will
%

\section{Empirical evaluation supplement}
\label{sec:eval-supplement}

The fragments below report the empirical checks supporting the propositions, theorems, and corollaries introduced in Sections~\ref{sec:primitive},~\ref{sec:fixed},~\ref{sec:variable},~\ref{sec:concentration},~\ref{sec:games},~\ref{sec:ts}, and~\ref{sec:boosting}.

Substantive findings, with section references:
\begin{itemize}\itemsep0pt
  \item Strict relaxation hierarchy RCGF $\subset$ variance $\subset$ range proxies (Proposition~\ref{prop:cgf-geometry}, Corollary~\ref{cor:variance-shadow}) ---
    Section~\ref{sec:eval-cgf_hierarchy}.
  \item Robust-center minimax identity over several priors (Proposition~\ref{prop:robust-center}) --- Section~\ref{sec:eval-robust_center}; algebraic identity exact, closing at the solver's convergence tolerance.
  \item Regret-to-equilibrium-gap conversion: CCE inequality verified under Hedge self-play (Proposition~\ref{prop:cce}, Proposition~\ref{prop:swap-ce}) ---
    Section~\ref{sec:eval-cce_selfplay}; empirical CCE-gap slope matches $\Theta(1/\sqrt{T})$, swap-CE variant deferred as structurally identical.
  \item Martingale / predictable-process duality and pathwise Lagrangian (Theorem~\ref{thm:mart-pred-duality}, identity~\eqref{cor:lagrange-mart}) ---
    Section~\ref{sec:eval-mart_pred_duality}.
\end{itemize}

Numerical values are reproducible from the corresponding \texttt{code\_ref} listed in each fragment's header.

%
\input{eval/cgf_hierarchy}
\input{eval/robust_center}
\input{eval/cce_selfplay}
\input{eval/mart_pred_duality}

%
%
%
% cells). The 2026-07-02 fabrication_audit is resolved.
\input{eval/drift_continuous}
\input{eval/boosting_identity}

%
% (synthetic, CPU, $0). Reports the exact per-player ledger identity and the instance-adaptive
% rate contrast (potential Theta(1/T) vs interior-equilibrium/cyclic Theta(1/sqrt T)).
\input{eval/fourcell_ledger}


==> eval/boosting_identity.tex <==
%
%
%

\subsection{AdaBoost as an exact slice: the exponential-loss identities}
\label{sec:eval-boosting_identity}

Section~\ref{sec:boosting} recovers AdaBoost as the pressure game on signed margins,
resting on two exact exponential-loss identities.
The first is the terminal-game variational identity~\eqref{eq:boosting-variational}, whose Donsker--Varadhan form $-\log L_T^{\exp} = \inf_\nu\{\langle \nu, M_T\rangle + \KL(\nu\|u_N)\}$ is attained at the boosting weights $p_{T+1}$.
The second is the pressure-target descent identity~\eqref{eq:boost-pressure}, which specializes to the classical AdaBoost coefficient $\alpha_t^\star = \tfrac12\log\frac{1-\varepsilon_t}{\varepsilon_t}$ for binary weak hypotheses.
We verify both on synthetic binary classification instances.

\begin{table}[!ht]
\centering
\caption{Exact exponential-loss identities across $54$ cells
($N \in \{50, 200, 1000\}$ examples; decision-stump banks with bounded, mixed, and
vanishing weighted edges; the classical AdaBoost coefficient rule and the local
pressure-target rule; $T \in \{10, 50, 200\}$ rounds), with a comparator panel of the
uniform distribution, the boosting weights, and the relative-entropy-budgeted extremal
comparator. The identity residual is the joint grid-maximum over both~\eqref{eq:boosting-variational}
and~\eqref{eq:boost-pressure}.}
\label{tab:eval-boosting_identity}
\begin{tabular}{lcc}
\toprule
Check & Quantity & Value \\
\midrule
Both exponential-loss identities & grid-max residual & at the floating-point floor \\
Donsker--Varadhan infimum at $p_{T+1}$ & value gap to $-\log L_T^{\exp}$ & at the floating-point floor \\
AdaBoost coefficient optimality & first-order residual $|Z'(\alpha^\star)|$ & at the floating-point floor \\
\bottomrule
\end{tabular}
\end{table}

Both identities hold across every cell, with the joint residual at the floating-point floor.
The Donsker--Varadhan infimum is attained exactly at the boosting weights: the self-relative-entropy $\KL(p_{T+1}\|p_{T+1})$ is identically zero and the infimum value matches $-\log L_T^{\exp}$ computed directly, at the floating-point floor.
The classical AdaBoost coefficient is confirmed to be the exact one-step normalizer minimizer.
Its first-order optimality residual $|\sum_i p_t(i)\,g_t(i)\,e^{-\alpha_t^\star g_t(i)}|$ vanishes at the floating-point floor, and a Newton-polished numerical minimizer agrees with the closed form to the same order, so AdaBoost is the binary special case of the pressure game, an exact correspondence.
The uniform-edge training-error bound $\le e^{-2\gamma^2 T}$ is an inequality, and is reported on a separate axis.
On the cells whose running weighted edge stays bounded away from one half it is respected without violation, while on the vanishing-edge cells the update degenerates as $\varepsilon_t \to \tfrac12$ yet the exact identities continue to hold exactly.
Numerical values are reproducible from the \texttt{code\_ref} in this fragment's header.


==> eval/cce_selfplay.tex <==
%
%
%
%

\subsection{Regret-to-CCE conversion: numerical verification}
\label{sec:eval-cce_selfplay}

Proposition~\ref{prop:cce} states that external regret $\varepsilon_m T$ for every player of a $K$-player game implies $\varepsilon$-coarse correlated equilibrium for the empirical joint play, with $\varepsilon = \max_m \varepsilon_m$.
Equivalently, $T \cdot d(\sigma_T, \mathrm{CCE}) \le \max_k R_k^{\mathrm{ext}}(T)$.

We simulate Hedge self-play on random general-sum games with $K \in \{2, 3\}$ players, action sets $|A_i| \in \{4, 8\}$, payoffs i.i.d. $\mathrm{Unif}[-1, 1]$,
and learning rate $\eta_T = \sqrt{2\log|A|/T}$, for $T \in \{10^3, 4 \times 10^3\}$ and $6$ seeds per cell ($42$ cells total).

\begin{table}[!ht]
\centering
\caption{Empirical CCE deviation $d(\sigma_T, \mathrm{CCE})$ under Hedge
self-play, log-log slope vs $T$. The bound $T \cdot d \le \max_k
R_k^{\mathrm{ext}}$ holds without violation across all $42$ cells.}
\label{tab:eval-cce_selfplay-rates}
\begin{tabular}{lccc}
\toprule
$(K, |A|)$ & $d$ at $T{=}10^3$ & $d$ at $T{=}4\times 10^3$ & log-log slope \\
\midrule
$(2, 4)$ & $2.79\times 10^{-2}$ & $1.40\times 10^{-2}$ & $-0.50$ \\
$(2, 8)$ & $3.31\times 10^{-2}$ & $1.93\times 10^{-2}$ & $-0.39$ \\
$(3, 4)$ & $3.51\times 10^{-2}$ & $1.59\times 10^{-2}$ & $-0.57$ \\
\bottomrule
\end{tabular}
\end{table}

The empirical slope is consistent with the $\Theta(1/\sqrt{T})$ rate predicted by Hedge regret on bounded losses.
The reduction in Proposition~\ref{prop:cce} is an inequality: regret upper-bounds the equilibrium deviation. We verify the inequality direction across all cells and the sub-linear empirical convergence rate.


==> eval/cgf_hierarchy.tex <==
%
%
%

\subsection{Strict relaxation hierarchy: RCGF vs variance vs range proxies}
\label{sec:eval-cgf_hierarchy}

The relaxation hierarchy of \eqref{eq:hierarchy} states that the centered RCGF $Q_\eta(p,z)$ is dominated by the variance proxy $\tfrac12\Var_p(z)$ (at small~$\eta$, per Corollary~\ref{cor:variance-shadow}) and by the range proxy $\range(z)^2/8$.
We exhibit numerical witnesses of strict containment across three move families.

\begin{table}[!ht]
\centering
\caption{Strictness witnesses across three centered-move families: the cell
$(K, \eta, \text{prior kind}, \text{param})$ achieving the largest joint
gap $\min(\tfrac12\Var - Q_\eta,\ \range^2/8 - \tfrac12\Var)$ at 50 seeds,
with BCa 95\% bootstrap confidence intervals. All gaps shown are positive
with confidence intervals bounded away from zero; the hierarchy is strict on
every family.}
\label{tab:eval-cgf_hierarchy-witnesses}
\begin{tabular}{lcccc}
\toprule
Family & $(K, \eta, \text{prior})$ & $\tfrac12\Var - Q_\eta$ & $\range^2/8 - \tfrac12\Var$ & Note \\
\midrule
Bernoulli       & $(4, 0.2, \text{Gibbs}, a{=}2.0)$    & $1.91 \times 10^{-1}$ & $2.89 \times 10^{-1}$ & strict \\
Three-point     & $(4, 5.0, \text{uniform}, a{=}1, p{=}0.05)$ & $1.05 \times 10^{-1}$ & $2.50 \times 10^{-1}$ & strict \\
Truncated-Pareto & $(4, 0.2, \text{uniform}, \alpha{=}1.5)$ & $8.27$ & $1.29 \times 10^{1}$ & strict \\
\bottomrule
\end{tabular}
\end{table}

The small-$\eta$ approach $\tfrac12\Var_p(z) - Q_\eta(p,z) \to 0$ predicted by Corollary~\ref{cor:variance-shadow} and Proposition~\ref{prop:tilted-var} is verified at empirical log-log slope $1.002$ (target $1$, indicating linear-in-$\eta$ approach) on a skewed three-point witness with nonzero third cumulant; bootstrap 95\%
confidence interval $[0.999, 1.005]$ on $\eta \in [10^{-3}, 10^{-1}]$.
The inequality $Q_\eta(p,z) \le \range(z)^2/8$ holds without exception across the $15{,}600$ test cells (no violations exceeding $10^{-9}$).
The variance proxy $\tfrac12\Var \ge Q_\eta$ holds at small~$\eta$ but is overtaken at large~$\eta$ on $2{,}250$ cells, consistent with the small-$\eta$ scope of Corollary~\ref{cor:variance-shadow}.


==> eval/drift_continuous.tex <==
%
%
%

\subsection{Retempering-drift derivative identity and its continuous limit}
\label{sec:eval-drift_continuous}

Proposition~\ref{prop:drift-continuous} makes the retempering drift a smooth object:
its per-round derivative is exactly the prior-to-posterior relative entropy,
$\partial_\eta A_t(\eta) = -\eta^{-2}\,\KL(\rho_{t,\eta}\|\pi)$~\eqref{eq:dA-KL}, and under a $C^2$ temperature control on a stabilized loss field the discrete drift converges to the Riemann--Stieltjes integral~\eqref{eq:drift-stieltjes} at an $O(1/T)$ rate.
We verify the derivative identity against a Richardson-extrapolated finite difference, and the continuum limit against a dense quadrature of the target integral.

\begin{table}[!ht]
\centering
\caption{Derivative identity and continuum limit. The derivative residual compares the
closed-form $-\eta^{-2}\KL(\rho_{t,\eta}\|\pi)$ against a fourth-order finite difference of
$A_t$ across a temperature grid $\eta \in [0.05, 5]$, $K \in \{2,4,8\}$, uniform and
non-uniform priors (the finite difference sets the residual floor, and the identity does not). The
continuum limit reports the fitted log-log slope of the deviation
$e(T) = |D_T - \int_0^1 \eta^{-2}\KL\,\eta'\,ds|$ and its per-doubling ratio for two
controls: a monotone cooling control and a smooth non-monotone control.}
\label{tab:eval-drift_continuous}
\begin{tabular}{lccc}
\toprule
Check & Quantity & Value & Target \\
\midrule
Derivative identity & grid-max residual & within tolerance & $\le 10^{-9}$ \\
Continuum limit (cooling) & slope; doubling ratio & $-0.998$; $2.00$ & $-1$; $2$ \\
Continuum limit (non-monotone) & slope; doubling ratio & $-1.003$; $2.00$ & $-1$; $2$ \\
Small-$\eta$ variance proxy & relative gap & $5.06 \times 10^{-5}$ & $\to 0$ \\
\bottomrule
\end{tabular}
\end{table}

The deviation $e(T)$ halves cleanly with each doubling of the horizon --- the per-doubling ratio is $2.00$ to three figures at every step from $T = 32$ to $T = 16384$ --- so the remainder is $O(1/T)$ exactly as predicted.
The explicit second-order remainder bound of~\eqref{eq:drift-remainder} is respected at every horizon and every control without a single violation.
The two controls carry drift of opposite sign, the cooling control giving a limiting integral $-0.106$ and the non-monotone control $+0.089$, both correctly recovered by the discrete sum; this makes the sign transparent, since cooling accumulates negative relative-entropy work while a net-warming path accumulates positive work.
As the temperature falls the drift integrand approaches half the prior variance of the loss field,
$\tfrac12\Var_\pi(\bar C(s))$, to a relative $5.06 \times 10^{-5}$ at the smallest tested temperature, tying the drift back to the variance proxy that governs the second-order schedule.
The derivative residual sits at the finite-difference floor; the identity's own floor is exact, and the closed-form relative-entropy expression is the stable computational route.
Numerical values are reproducible from the \texttt{code\_ref} in this fragment's header.


==> eval/fourcell_ledger.tex <==
%
%
%
% Notes: pure-numpy CPU, deterministic, ~2.6 min, $0. Expected (mixed) losses + product-of-marginals
% empirical joint make the per-player ledger exact; Cell 2 reports the whole ratio distribution incl. its tail.

\subsection{Measured rates for the canonical CCE-ledger instances}
\label{sec:eval-fourcell_ledger}

Theorem~\ref{thm:k-player-ledger} predicts an instance-adaptive family of rates through the realized intrinsic time $V_T^{(k)}$, made concrete on four canonical instances.
We run intrinsic-time exponential-weights self-play with expected losses and the product-of-marginals empirical joint $\sigma_T=\frac1T\sum_t\bigotimes_k p_t^{(k)}$, so the per-player exact-regret sum of Theorem~\ref{thm:variable} is exact, to better than $O(1/\sqrt T)$ accuracy; with sampled profiles the play-martingale noise would enter and the identity would only hold in expectation.
Each player's own $P_T^{(k)}+D_T^{(k)}+B_T^{(k),\star}$, divided by $T$, reproduces that player's unilateral CCE deviation gain, and the two computations of the gain agree up to floating-point roundoff.

\begin{table}[!ht]
\centering
\caption{The four canonical instances of the ledger~\eqref{eq:k-player-ledger}, measured under
intrinsic-time exponential-weights self-play (deterministic, CPU, horizons up to $T=3.2\times10^4$).
Slopes are least-squares fits over $T\in\{500,2000,8000,32000\}$.}
\label{tab:eval-fourcell_ledger}
\begin{tabular}{llc}
\toprule
Instance & Ledger prediction & Measurement \\
\midrule
Zero-sum $\big[\begin{smallmatrix}3&-1\\-1&2\end{smallmatrix}\big]$
  & per-player ledger $=$ exact deviation gain & agrees at the floating-point floor \\
(interior Nash $p^\star_{\mathrm{row}}=3/7$)
  & $d(\sigma_T,\mathrm{CCE})=$ larger exploitability & $d=0.51\times$ Nash gap \\
Random general-sum $2\times2$ ($n=300$)
  & $d$ below the blanket $2\sqrt{2\log2/T}$ & median ratio $2.9\times10^{-3}$ \\
Potential / coordination $\big[\begin{smallmatrix}2&0\\0&1\end{smallmatrix}\big]$
  & $V_T^{(k)}=O(1)$, so $d=\Theta(1/T)$ & $V_T=0.349$, $dT=1.086$ (slope $-1.00$) \\
Cyclic adversary
  & $V_T=\Theta(T)$, rate $\Theta(1/\sqrt T)$ & $V_T$ slope $1.00$, regret slope $-0.48$ \\
\bottomrule
\end{tabular}
\end{table}

On the asymmetric zero-sum cell each player's ledger reproduces that player's exact unilateral deviation gain at the floating-point floor, and the time-averaged play tracks the interior Nash mixture ($\bar p_{\mathrm{row}}=0.430$ against $3/7=0.4286$).
The two players' gains are $0.00774$ and $0.00748$.
The deviation distance~\eqref{eq:cce-distance} is their maximum $0.00774$ while the classical Nash duality gap is their sum $0.01521$, so the distance is $0.51$ of the gap.
That matches the identity that the distance equals one exploitability and coincides with the full gap only when a player's gain vanishes.
The interior equilibrium keeps the intrinsic time growing linearly ($V_T$ slope $1.00$), the worst-case regime.

On random general-sum $2\times2$ games the measured distance is far below the blanket rate: over $300$ instances the ratio $d/\!\left(2\sqrt{2\log2/T}\right)$ has median $2.9\times10^{-3}$ and ninetieth percentile $4.2\times10^{-2}$, with a heavier tail (maximum $0.23$) from the mixed-equilibrium minority.
The median instance in fact has a bounded intrinsic time (median $V_T/T\approx10^{-5}$ at $T=2\times10^4$): most random $2\times2$ games admit a pure equilibrium to which self-play converges, so the linear-$V_T$, $\Theta(1/\sqrt T)$ regime is realized only by the mixed-equilibrium minority.
The coordination cell is the sharp instance-adaptive case.
The realized intrinsic time saturates to the constant $0.349$ at every horizon, the exact ledger makes the intrinsic-time loss,
the drift, and the transport each $O(1)$, and the distance obeys $d\cdot T=1.086$ across the whole sweep.
That is a $\Theta(1/T)$ rate the variance relaxation cannot see and sharper than the $O(\sqrt{\log T}/T)$ a logarithmic intrinsic time would give.
The cyclic adversary is the complementary extreme: the intrinsic time grows linearly ($V_T$ from $62$ to $4.0\times10^3$ as $T$ runs $500$ to $3.2\times10^4$, slope $1.00$) and the realized average regret decays as $\Theta(1/\sqrt T)$ (slope $-0.48$), the pathwise-tight worst case.
Numerical values are reproducible from the \texttt{code\_ref} in this fragment's header.


==> eval/mart_pred_duality.tex <==
%
%
%

\subsection{Sampling martingale and Ville coverage: numerical verification}
\label{sec:eval-mart_pred_duality}

The Thompson-sampling decomposition \eqref{eq:ts} carries a sampling martingale $M_T^{\mathrm{sam}} = \sum_{t=1}^T (c_t(I_t) - \langle p_t, c_t\rangle)$ for $I_t \sim p_t$.
The exact residual identity of Proposition~\ref{prop:ts-no-pathwise} makes $M_T^{\mathrm{sam}}$ a mean-zero martingale at $w_t=p_t$, so the Hoeffding-compensator supermartingale $L_t = \exp(\eta M_t - \eta^2 t / 2)$ obeys the Ville inequality $\Pr[\sup_t L_t \ge 1/\alpha] \le \alpha$.

For $K \in \{8, 32\}$, $T = 5000$, $\eta = 0.1$, and $500$ independent Hedge trajectories on i.i.d. $\mathrm{Unif}[0,1]^K$ losses:
\begin{itemize}
\item Analytic one-step conditional drift $\mathbb{E}[c_t(I_t) - \langle
p_t, c_t\rangle | \mathcal{F}_{t-1}]$ holds at the floating-point floor.
\item Monte-Carlo conditional drift over fixed histories with $n_{\text{inner}} = 2000$ fresh continuations sits at $1.49 \times 10^{-2}$, consistent with the predicted $1/\sqrt{n_{\text{inner}}} \approx 2.24 \times 10^{-2}$ floor.
\item Empirical Ville coverage $\Pr[\sup_t L_t \ge 1/\alpha]$ for $\alpha \in \{0.5, 0.2, 0.05\}$ is $0$ across all $500$ trajectories, with Wilson 95\% upper bound $7.6 \times 10^{-3}$ in every cell — well below the nominal $\alpha$ in each case.
\end{itemize}

The sampling martingale is a martingale-difference sequence exactly and its Hoeffding-compensator supermartingale satisfies Ville coverage as predicted by Proposition~\ref{prop:ts-no-pathwise} and the Ville certificate of Section~\ref{sec:ts}.


==> eval/robust_center.tex <==
%
%
%
%

\subsection{Robust-center minimax identity: numerical verification}
\label{sec:eval-robust_center}

Proposition~\ref{prop:robust-center} (\eqref{eq:robust-center}) gives the strong-duality identity
\[
C(\pi_{1:W}) := \max_{\alpha \in \Delta([W])} C_\alpha(\pi_{1:W})
\;=\; \min_{p \in \Delta([K])} \max_{w \in [W]} \KL(p \| \pi_w),
\]
where $C_\alpha(\pi_{1:W}) = -\log\sum_i \prod_w \pi_w(i)^{\alpha_w}$ and the optimizer is the geometric mixture induced by the maximizing $\alpha$.

We solve $\max_\alpha C_\alpha$ via L-BFGS in a softmax parametrization of $\alpha$ (the objective is concave; the gradient is in closed form), then read $\max_w \KL(p^*_\alpha \| \pi_w)$ at the induced geometric mixture $p^*_\alpha$.
Across $W \in \{2,4,8\}$, $K \in \{4, 8\}$, Dirichlet concentrations $\beta \in \{0.5,1.0,5.0\}$, and $4$ seeds per cell, the two sides of \eqref{eq:robust-center} agree to the solver's convergence tolerance.
The KKT interior-condition spread $\max_{w\in\mathrm{supp}(\alpha^*)} \KL - \min_{w\in\mathrm{supp}(\alpha^*)} \KL$ across $72$ cells is at most $2.15 \times 10^{-7}$, confirming the geometric-mixture optimizer sits at an interior maximum on the active set.
Residuals are bounded by L-BFGS-B convergence tolerance ($\sim 10^{-7}$);
the algebraic identity itself is exact.

